Compass: A Decentralized Scheduler for Latency-Sensitive ML Workflows

We consider ML query processing in distributed systems where GPU-enabled workers coordinate to execute complex queries: a computing style often seen in applications that interact with users in support of image processing and natural language processing. In such systems, coscheduling of GPU memory management and task placement represents a promising opportunity. We propose Compass, a novel framework that unifies these functions to reduce job latency while using resources efficiently, placing tasks where data dependencies will be satisfied, collocating tasks from the same job (when this will not overload the host or its GPU), and efficiently managing GPU memory. Comparison with other state of the art schedulers shows a significant reduction in completion times while requiring the same amount or even fewer resources. In one case, just half the servers were needed for processing the same workload.

==> 9_workflows.tex <==
\remove{
% Moved back to Section2
\newpage
\section*{Appendix A: Experimental Workflows} 
\label{sec:Workflows}
To illustrate the approach, we use the {\staticgraph} this notation to express a representative group of applications arising in ML language processing and image understanding.  Our experimental section used these workflows as its scheduling target.

The first workflow in Figure~\ref{fig:translation} arises in an application for real-time multi-language translations of the kind supporting multilingual remote diagnosis~\cite{multilanguageOCR} or multilingual product planning, for example during a Teams or Zoom meeting with attendees who prefer captions in their native languages.  We want the various translations to be rendered simultaneously, hence the pipeline first aggregates all the translation results and then outputs them as a set. Notice that the vertices in the {\staticgraph} designate the MLs used at each stage. 
 The input vertex employs an Open Pre-trained Transformer (OPT) model~\cite{opt}, facebook/opt-1.3b. The role of this vertex is to create a uniform representation of the points the speaker is making. 
 Next the various translation components create language-specific summarizations from this shared intermediary object using encoder-decoder transformer framework models (specifically,  using Marian~\cite{marian, en_fr_model} for French and mt5~\cite{mt5, zh_ja_en_model} for Chinese and Japanese). Notice that although mt5 plays two roles, it requires just one model \-- the target language is specified as part of the prompt.

The second workflow (Figure~\ref{fig:readimg}) arises in an application that auto-captions images, for example in the education scenario described in~\cite{education} where a smart pad describes an image in a text and reads it out loud as a child pages through a book. The {\staticgraph} employs the ViT-GPT2 model~\cite{vit-gpt2, vit-gpt2-model} for automated captioning. Next, the text description is subsequently processed by ESPnet~\cite{espnet} to vocalize the text while BART~\cite{bart} runs in parallel to perform a content check, ensuring that only child-safe results are generated. The {\staticgraph} terminates with a node that aggregates the two outputs and emits either the caption and vocalization, or a null tuple if the caption fails content checking.

The third workflow (Figure~\ref{fig:dialogue}) is intended to answer a posed question, and might be 
 deployed in a Virtual Personal Assistants(VPA)~\cite{personal_assistant}. The intent is to respond to user inquiries while ignoring adversarial questions and inhibiting  answers that might be perceived as argumentative, angry or snarky: concerns identified in~\cite{content_signal}. Here, the questions are answered using the OPT model (the same one used in the translation workflow in Figure~\ref{fig:translation}), but with different prompts employed to "shape" the desired output. Content checking functionality is performed by BART~\cite{bart}, as was the case for the second workflow, but with prompts that characterize the user as an adult rather than a child.

The fourth workflow (Figure~\ref{fig:3dperception}) is an image processing {\staticgraph} used for a task that might arise in in a driving assistance unit within a car navigating a smart city~\cite{depth_estimation} or in household tasks where a mix of image recognition and depth perception are required~\cite{conceptfusion}. We see two models in this {\staticgraph}. Object detection is performed by the DEtection TRansformer (DETR)~\cite{detr} model; object depth estimation from a single image is performed by a hierarchical transformer encoder-decoder model~\cite{glpn}. The info aggregation vertex combines the outputs from object detection and depth estimation. 

Notice that while these {\staticgraph}s could be applied on a per-event basis, we could also instantiate an event-processing stream by precomputing task placements and preallocating resources, after which a series of events could be routed through each stream without needing to repeat scheduling decisions each time. This paper limits itself to scenarios in which each new event triggers a scheduling decision.



}



\remove{
\section*{Appendix B: Centralized vs Decentralized Scheduling} 
\label{sec:centralizedVSdecentralized}


% centralized

% bottleneck, 
% overhead to data transfer,
% dynamic adjustment at the last step is more precise

% it receives the worker information in the same way as decentralized. The workload prediction may not work if the workload is changing and especially the ML runtime has high variation

Compass uses a decentralized scheduling algorithm for several reasons: this eliminates a central bottleneck (at the small cost of an overhead to share metadata needed for scheduling decisions), and also eliminates the latency of "consulting" the central scheduler on every scheduling event.  However, by making this choice we lose the obvious advantages of a centralized approach: all scheduling decisions are made in one place, and concurrent decisions use identical information about cluster state.  There are cases when this centralization can be advantageous.  For example, when the request rates are relatively stable or with certain known distribution that can be captured by scheduler, centralized scheduler can allocate the models to worker's Compass cache accordingly. However, Compass targets a setting where workflows are known but the load and distribution of requests is not predictable. 

A second case where the centralized scheduler has an advantage is when concurrent task assignments must occur: a centralized solution will place the tasks in a coordinated, consistent way, whereas a decentralized one might accidentally overload some worker, forcing a reassignment of one or more tasks.  In our experiments, this case did not arise often, and did not result in any measurable degradation of performance.  

%Decentralized scheduler has some benefits that made it a good fit for our scenario. First decentralized scheduler have the natural first step load-balancing, by sending the first task to one of the worker's scheduler, it can have shorted queuing delay at scheduling queue, comparing to centralized scheduler, which could be a bottleneck under heavy load and have longer queue. And if the local worker is scheduled to be executing the first task, it can also avoid the data transfer time of the first task.   The large scale ML tasks have runtimes with high variation. This means the prediction of runtimes estimated by the centralized scheduler loss its precision, but to rely on the dynamic task adjustment in the same way as Compass. 


}

